On Label Shift in Domain Adaptation via Wasserstein Distance

We study the label shift problem between the source and target domains in general domain adaptation (DA) settings. We consider transformations transporting the target to source domains, which enable us to align the source and target examples. Through those transformations, we define the label shift between two domains via optimal transport and develop theory to investigate the properties of DA under various DA settings (e.g., closed-set, partial-set, open-set, and universal settings). Inspired from the developed theory, we propose Label and Data Shift Reduction via Optimal Transport (LDROT) which can mitigate the data and label shifts simultaneously. Finally, we conduct comprehensive experiments to verify our theoretical findings and compare LDROT with state-of-the-art baselines.

==> LDROT.tex <==
Inspired by the developed theory in Section~\ref{sec:label_shift_optimal_transport},
in this section we propose a novel DA approach, named \textbf{\emph{L}}\emph{abel
and }\textbf{\emph{D}}\emph{ata Shift }\textbf{\emph{R}}\emph{eductions
via }\textbf{\emph{O}}\emph{ptimal }\textbf{\emph{T}}\emph{ransport}
(LDROT), that aims to reduce both data and label shifts simultaneously.
%\vspace{-2mm}


\subsection{Objective function of LDROT}

We consider the source classifier $h^{S}=\bar{h}^{S}\circ g$ and
the target classifier $h^{T}=\bar{h}^{T}\circ g$. The pathway of
our method consists of three losses, which are as follows:

(i) \textit{Standard loss $\mathcal{L}^{S}$}: We train the source
classifier $h^{S}$ on the labeled source data by minimizing the loss
$\mathcal{L}^{S}:=\mathcal{L}\left(h^{S},f^{S},\mathbb{P}^{S}\right)$;

(ii) \textit{Shifting loss $\mathcal{L}^{shift}$}: Furthermore, to
mitigate both label and data shifts, we propose to further regularize
the loss $\mathcal{L}^{S}$ by $\mathcal{L}^{shift}:=\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$,
where the ground metric $d$ is defined as 
\begin{equation}
d\left(\bz^{S},\bz^{T}\right)=\lambda\cdot d_{X}\left(g\left(\bx^{S}\right),g\left(\bx^{T}\right)\right)+d_{Y}\left(h^{S}\left(\bx^{S}\right),h^{T}\left(\bx^{T}\right)\right),\label{eq:d_metric}
\end{equation}
where $\bz^{S}=\left(\bx^{S},h^{S}\left(\bx^{S}\right)\right)$ with
$\bx^{S}\sim\mathbb{P}^{S}$ and $\bz^{T}=\left(\bx^{T},h^{T}\left(\bx^{T}\right)\right)$
with $\bx^{T}\sim\mathbb{P}^{T}$;

(iii) \textit{Clustering loss $\mathcal{L}^{clus}$}: Finally, to
boost the generalization ability of $h^{T}$, we enforce the clustering
assumption \citep{chapelle2005semi} to enable $h^{T}$ giving the
same prediction for source and target examples on the same cluster.
To employ the clustering assumption \citep{shu2018a}, we use Virtual
Adversarial Training (VAT) \citep{VAT} in conjunction with minimizing
the entropy of prediction \citep{grandvalet2015entropy}: $\mathcal{L}^{clus}:=\mathcal{L}^{ent}+\mathcal{L}^{vat}$
with{\small{}
\begin{align*}
\mathcal{L}^{ent} & =\mathbb{E}_{\mathbb{P}^{T}}\left[\mathbb{H}\left(h^{T}\left(g\left(\bx\right)\right)\right)\right], \\
\mathcal{L}^{vat} & =  \mathbb{E}_{0.5\mathbb{P}^{S}+0.5\mathbb{P}^{T}}\left[\text{max }_{\bx'\in B_{\theta}\left(\bx\right)}D_{KL}\left(h^{T}\left(g\left(\bx\right)\right),h^{T}\left(g\left(\bx'\right)\right)\right)\right],
\end{align*}
} where $D_{KL}$ represents a Kullback-Leibler divergence, $\theta$
is a very small positive number, $B_{\theta}\left(\bx\right):=\left\{ \bx':\norm{\bx'-\bx}_{2}<\theta\right\} $,
and $\mathcal{\mathbb{H}}$ specifies the entropy.

Combining the above losses, we arrive at the following objective function
of LDROT. 
\begin{align}
\inf_{g,\bar{h}^{S},\bar{h}^{T}}\{\mathcal{L}^{S}+\alpha\mathcal{L}^{shift}+\beta\mathcal{L}^{clus}\},\label{eq:LDROT_loss}
\end{align}
where $\alpha,\beta>0$. In addition, we use the target classifier
$h^{T}$ to predict target examples.

\textbf{Remark on the shifting term:} We now explain why including
the shifting term $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
supports to reduce label and data shifts. First, we have the following
inequality whose proof can be found in Appendix \ref{sec:proof_remaining_results}:
\begin{equation}
\mathcal{W}_{d_{X}}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)=\mathcal{W}_{d_{X}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)\leq\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)\label{eq:data_shift_bound}
\end{equation}
since $d_{X}\leq d$. 

Therefore, by including the shifting term $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$,
we aim to reduce $\mathcal{W}_{d_{X}}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)$,
which is useful for reducing the data shift on the latent space.

Second, we find that $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)\leq\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
since $d_{Y}\leq d$. The inequality (i) in Proposition \ref{proposition:properties_labelshift}
suggests that reducing the label shift $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
helps to reduces the loss on the target domain, therefore increasing
the quality of our DA method.  Finally, by including $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$,
we aim to simultaneously reduce both terms $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
and $\mathcal{W}_{d_{X}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$,
which is equal to $\mathcal{W}_{d_{X}}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)$.
That step helps reduce the data shift between $g\#\mathbb{P}^{S}$and
$g\#\mathbb{P}^{T}$, while forcing $h^{T}$ to mimic $h^{S}$ for
predicting well on the target domain via reducing the label shift
$\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$.
%\vspace{-2mm}


\subsection{Training procedure of LDROT}

We now discuss a few important aspects of the training procedure of
LDROT.

\vspace{0.5 em}
\noindent
\textbf{Similarity-aware version of the ground metric $d$:} The weight
$\lambda$ in the ground metric $d$ in Eq.~(\ref{eq:d_metric})
represents the matching extent of $g\left(\bx^{T}\right)$ and $g\left(\bx^{S}\right)$.
Ideally, we would like to replace this fixed constant $\lambda$ by
varied weights $\bw\left(\bx^{S},\bx^{T}\right)$ in such a way that
$\bw\left(\bx^{S},\bx^{T}\right)$ is high if $\bx^{T}$ and $\bx^{S}$
share the same label and low otherwise. However, it is not possible
because the label of $\bx^{T}$ is unknown. As an alternative, it
appears that if we can have a good way to estimate the pairwise similarity
$s\left(\bx^{S},\bx^{T}\right)$ of $\bx^{T}$ and $\bx^{S}$, $s\left(\bx^{S},\bx^{T}\right)$
seems to be high if $\bx^{T}$ and $\bx^{S}$ share the same label
and low if otherwise. Based on this observation, we instead propose
using a similarity-aware version of metric $d$ as follows: 
\[
\bar{d}\left(\bz^{S},\bz^{T}\right)=\bw\left(\bx^{S},\bx^{T}\right)d_{X}\left(g\left(\bx^{S}\right),g\left(\bx^{T}\right)\right)+d_{Y}\left(h^{S}\left(\bx^{S}\right),h^{T}\left(\bx^{T}\right)\right),
\]
where the weight $\bw\left(\bx^{S},\bx^{T}\right)$ is estimated based
on $s\left(\bx^{S},\bx^{T}\right)$. 

\vspace{0.5 em}
\noindent
\textbf{Entropic regularized version of shifting term:} Since computing
directly the shifting term $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
is expensive, we use the entropic regularized version of $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
instead, which we denote $\mathcal{W}_{d}^{\epsilon}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
where $\epsilon$ is a positive regularized term (Detailed definition
and discussion of the entropic regularized Wasserstein metric is in
Appendix A). The dual-form~\citep{stochastic_ws} of that entropic
regularized term with respect to the ground metric $\bar{d}$ admits
the following form:{\footnotesize{}
\begin{equation}
\max_{\phi}\Biggl\{\frac{1}{N_{S}}\sum_{i=1}^{N_{S}}\phi\left(g\left(\bx_{i}^{S}\right)\right)-\frac{\epsilon}{N_{T}}\sum_{j=1}^{N_{T}}\Biggl[\log\Biggl(\frac{1}{N_{S}}\sum_{i=1}^{N_{S}}\exp\Biggl\{\frac{\phi\left(g\left(\bx_{i}^{S}\right)\right)-\bar{d}\left(\bz_{i}^{S},\bz_{j}^{T}\right)}{\epsilon}\Biggr\}\Biggr)\Biggr]\Biggr\},\label{eq:entropic_WS-1}
\end{equation}
}where $\phi$ is a neural net named the Kantorovich potential network,
$\left\{ \left(\bx_{i}^{S},y_{i}^{S}\right)\right\} _{i=1}^{N_{S}}$and
$\left\{ \bx_{i}^{T}\right\} _{i=1}^{N_{T}}$ are source and target
data, $\bz_{i}^{S}=(\bx_{i}^{S},h^{S}(\bx_{i}^{S}))$, $\bz_{j}^{T}=(\bx_{j}^{T},h^{T}(\bx_{j}^{T}))$,
and $\bw_{ij}=\bw\left(\bx_{i}^{S},\bx_{j}^{T}\right)$.

\vspace{0.5 em}
\noindent
\textbf{Evaluating the weights $\bw_{ij}$:} The weights $\bw_{ij}$
are evaluated based on the similarity scores $s_{ij}:=s\left(\bx_{i}^{S},\bx_{j}^{T}\right)$.
Basically, we train from scratch or fine-tune a pre-trained deep net
(e.g., ResNet~\citep{he2016resnet}) using source dataset with labels
and compute cosine similarity of latent representations $\boldsymbol{r}_{j}^{T}$
and $\boldsymbol{r}_{i}^{S}$ of $\bx_{j}^{T}$ and $\bx_{i}^{S}$
as $s_{ij}=s\left(\bx_{i}^{S},\bx_{j}^{T}\right)=\text{cosine-sim}\left(\boldsymbol{r}_{i}^{S},\boldsymbol{r}_{j}^{T}\right).$

To ease the computation, we estimate the weights $\bw_{ij}$ according
to source and target batches. Specifically, we consider a balanced
source batch of $Mb$ source examples (i.e., $M$ is the number of
classes and $b$ is source batch size for each class). For a target
example $\bx_{j}^{T}$ in the target batch, we sort the similarity
array $\left[s_{ij}\right]_{i=1}^{Mb}$ in an ascending order. Ideally,
we expect that the similarity scores of the target example $\bx_{j}^{T}$
and the source examples $\bx_{i}^{S}$ with the same class as $\bx_{j}^{T}$
(i.e., totally we have $b$ of theirs) are higher than other similarity
scores in the current source batch. Therefore, we find $\mu_{i}$
as the $\frac{M-1}{M}$-percentile of the ascending similarity array
$\left[s_{ij}\right]_{i=1}^{Mb}$ and compute the weights as $\bw_{ij}=\exp\left\{ \frac{\bs_{ij}-\mu_{i}}{\tau}\right\} $
with a temperature variable $\tau$. It is worth noting that this
weight evaluation strategy assists us in \emph{sharpening} and \emph{contrasting}
the weights for the pairs in the similar and different classes. More
specifically, for the pairs in the same classes, $\bs_{ij}$ tend
to be bigger than $\mu_{i}$, whilst for the pairs in different classes,
$\bs_{ij}$ tend to be smaller than $\mu_{i}$. Hence, with the support
of exponential form and temperature variable $\tau$, $\bw_{ij}$
for the pairs in the same classes tend to be higher than those for
the pairs in different classes. 

\paragraph{Comparing to DeepJDOT \citep{damodaran2018deepjdot}: }

The $\mathcal{W}_{d}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
with $d=\lambda d_{X}+d_{Y}$ was investigated in DeepJDOT \citep{damodaran2018deepjdot}. However,
ours is different from that work in some aspects: (i) \emph{similarity
based dynamic weighting}, (ii) \emph{clustering loss} for enforcing
clustering assumption for target classifier, and (iii) \emph{entropic
dual form} for training rather than Sinkhorn as in \cite{damodaran2018deepjdot}. More analysis of  LDROT can be found in Section \ref{more_analysis}.

\begin{table}[t!]
\centering{} %\vspace{-5mm}
 \caption{Classification accuracy (\%) on Office-31 dataset for unsupervised
DA (ResNet-50).\label{tab:office31-dataset-1}}
\resizebox{0.6\columnwidth}{!}{\centering\setlength{\tabcolsep}{2pt}%%
\begin{tabular}{cccccccc}
\hline 
Method  & A$\rightarrow$W  & A$\rightarrow$D  & D$\rightarrow$W  & W$\rightarrow$D  & D$\rightarrow$A  & W$\rightarrow$A  & Avg\tabularnewline
\hline 
ResNet-50 \citep{he2016resnet}  & 70.0  & 65.5  & 96.1  & 99.3  & 62.8  & 60.5  & 75.7\tabularnewline
DeepCORAL \citep{sun2016coral}  & 83.0  & 71.5  & 97.9  & 98.0  & 63.7  & 64.5  & 79.8\tabularnewline
DANN \citep{ganin2016domain}  & 81.5  & 74.3  & 97.1  & 99.6  & 65.5  & 63.2  & 80.2\tabularnewline
ADDA \citep{tzeng2017ADDA}  & 86.2  & 78.8  & 96.8  & 99.1  & 69.5  & 68.5  & 83.2\tabularnewline
CDAN \citep{long2018cdan}  & 94.1  & 92.9  & 98.6  & \textbf{100.0}  & 71.0  & 69.3  & 87.7\tabularnewline
TPN \citep{pan2019tpn}  & 91.2  & 89.9  & 97.7  & 99.5  & 70.5  & 73.5  & 87.1\tabularnewline
SAFN \citep{xu2019sfan}  & 90.1  & 90.7  & 98.6  & 99.8  & 73.0  & 70.2  & 87.1\tabularnewline
rRevGrad+CAT \citep{deng2019cluster}  & 94.4  & 90.8  & 98.0  & \textbf{100.0}  & 72.2  & 70.2  & 87.6\tabularnewline
DeepJDOT \citep{damodaran2018deepjdot}  & 88.9  & 88.2  & 98.5  & 99.6  & 72.1  & 70.1  & 86.2\tabularnewline
ETD \citep{li2020enhanceOT}  & 92.1  & 88.0  & \textbf{100.0}  & \textbf{100.0}  & 71.0  & 67.8  & 86.2\tabularnewline
RWOT \citep{xu2020reliable}  & 95.1  & 94.5  & 99.5  & \textbf{100.0}  & 77.5  & 77.9  & 90.8\tabularnewline
\hline 
\textbf{LDROT}  & \textbf{95.6}  & \textbf{98.0}  & 98.1  & \textbf{100.0}  & \textbf{85.6}  & \textbf{84.9}  & \textbf{93.7}\tabularnewline
\hline 
\end{tabular}}%\vspace{-3mm}
 
\end{table}
\begin{figure}[t!]
\begin{centering}
\subfloat[{{Closed-set setting with\protect \protect \\
 ~~$\mathcal{Y}^{S}=\mathcal{Y}^{T}=[9]$.}}]{\includegraphics[width=0.5\textwidth]{figures/1_uda}

}\subfloat[{{Open-set setting with \protect \protect \\
 ~~$\mathcal{Y}^{S}=[6]$, $\mathcal{Y}^{T}=[9]$.}}]{\includegraphics[width=0.5\textwidth]{figures/3_oda}

} \\
\subfloat[{{Partial-set setting with \protect \protect \\
 ~~$\mathcal{Y}^{S}=[9]$, $\mathcal{Y}^{T}=[6]$.}}]{\includegraphics[width=0.5\textwidth]{figures/2_pda}

}\subfloat[{{Universal setting with $\mathcal{Y}^{S}=[3]\cup\left\{ 4,5,6\right\} $, \protect \protect \\
 ~~$\mathcal{Y}^{T}=[3]\cup\left\{ 7,8,9\right\} $. }}]{\includegraphics[width=0.5\textwidth]{figures/4_unida}

}
\par
\end{centering}
\centering{} %\vspace{-2mm}
 \caption{Label shift estimation for various settings of DA when the source
data set SVHN and the target data set is MNIST. Here, we denote $[C]:=\left\{ 0,1,...,C\right\} $
for a positive integer number $C$.\label{fig:label_shift_estimation}}
%\vspace{-4mm}
\end{figure}



==> LabelShiftwithWS.tex <==

\subsection{Preliminaries}

\textbf{Notation.} For a positive integer $n$ and a real number $p\in[1,\infty)$,
$[n]$ indicates the set $\{1,2,\ldots,n\}$ while $\|x\|_{p}$ denotes
the $l_{p}$-norm of a vector $x\in\mathbb{R}^{n}$. Let $\mathcal{Y}^{S}$
and $\mathcal{Y}^{T}$ be the label sets of the source and target
domains that have $M^{S}:=\left|\mathcal{Y}^{S}\right|$ and $M^{T}:=\left|\mathcal{Y}^{T}\right|$
elements, respectively. Meanwhile, $\mathcal{Y}=\mathcal{Y}^{S}\cup\mathcal{Y}^{T}$
stands for the label set of both domains which has the cardinality
of $M:=\left|\mathcal{Y}\right|$. Subsequently, we denote $\mathcal{Y}_{\Delta}$,
$\mathcal{Y}_{\Delta}^{S}$, and $\mathcal{Y}_{\Delta}^{T}$ as the
simplices corresponding to $\mathcal{Y},\mathcal{Y}^{S}$, and $\mathcal{Y}^{T}$
respectively. Finally, let $f^{S}\left(\cdot\right)\in\mathcal{Y}_{\simplex}$
and $f^{T}\left(\cdot\right)\in\mathcal{Y}_{\simplex}$ be the labeling
functions of the source and target domains, respectively, by filling
zeros for the missing labels.

We now examine a general supervised learning setting. Consider a hypothesis
$h\left(\cdot\right)\in\mathcal{Y}_{\triangle}$ in a hypothesis class
$\mathcal{H}$ and a labeling function $f\left(\cdot\right)\in\mathcal{Y}_{\triangle}$
where $\mathcal{Y}_{\triangle}:=\left\{ \bpi\in\mathbb{R}^{M}:\norm{\bpi}_{1}=1\,\text{and \ensuremath{\bpi\geq\bzero}}\right\} $.
Let $d_{Y}$ be a metric over $\mathcal{Y}_{\triangle}$, we further
define a general loss of the hypothesis $h$ with respect to the labeling
function $f$ and the data distribution $\mathbb{P}$ as: $\mathcal{L}\left(h,f,\mathbb{P}\right):=\int d_{Y}\left(h\left(\bx\right),f\left(\bx\right)\right)\mathrm{d}\mathbb{P}\left(\bx\right)$.

Next, we consider a domain adaptation setting in which we have source
space $\mathcal{X}^{S}$ endowed with a distribution $\mathbb{P}^{S}$
and the density function $p^{S}\left(\bx\right)$, and a target space
$\mathcal{X}^{T}$ endowed with a distribution $\mathbb{P}^{T}$ and
the density function $p^{T}\left(\bx\right)$. We examine various
DA settings based on the labels of source and target domains including
(1) \emph{closed-set DA}: $\mathcal{Y}^{S}=\mathcal{Y}^{T}$, (2)
\emph{open-set DA}: $\mathcal{Y}^{S}\subset\mathcal{Y}^{T}$, (3)
\emph{partial-set DA}: $\mathcal{Y}^{T}\subset\mathcal{Y}^{S}$, and
(4) \emph{universal DA}: $\mathcal{Y}^{S}\subsetneq\mathcal{Y}^{T}$
and $\mathcal{Y}^{T}\subsetneq\mathcal{Y}^{S}$. 
\begin{figure}[!t]
\centering{}%\vspace{-1mm}
\includegraphics[width=0.75\textwidth]{Illustration.png}%\vspace{-3mm}
\caption{An illustration of our label shift definition. We employ a transformation
$L:L\#\mathbb{P}^{T}=\mathbb{P}^{S}$ to align two domains. The white/square
points $L\left(\protect\bx^{T}\right)$ on the source domain correspond
to the white/square points $\protect\bx^{T}$ on the target domain.
We measure $d_{Y}\left(d_{Y}\left(f^{T}\left(\protect\bx^{T}\right),f^{S}\left(L\left(\protect\bx^{T}\right)\right)\right)\right)$
and define the label shift w.r.t. $L$ as $LS\left(S,T;L\right):=\mathbb{E}_{\mathbb{P}^{T}}\left[d_{Y}\left(f^{T}\left(\protect\bx^{T}\right),f^{S}\left(L\left(\protect\bx^{T}\right)\right)\right)\right]$.
Finally, we take infimum over all valid $L$ to define the label shift
between two domains.\label{fig:motivation_LS}}
%\vspace{-7mm}
\end{figure}

\subsection{Background on label shift}

Together with data shift, the study of label shift is important for
a general DA problem. However, due to the occurrence of data shift,
it is challenging to formulate label shift in a general DA setting.
Recent works \citep{pmlr-v80-lipton18a,unified_labelshift_NEURIPS2020}
have studied label shift for the anti-causal setting in which an intervention
on \emph{$p(y)$} induces the shift, but the process generating $\bx$
given $y$ is fixed, i.e., $p^{S}\left(\bx\mid y\right)=p^{T}\left(\bx\mid y\right)$.
In spite of being useful in some specific cases, the anti-causal setting
is restricted and cannot represent data shift broadly because the
source data distribution $p^{S}\left(\bx\right)$ and the target data
distribution $p^{T}\left(\bx\right)$ are simply just two different
mixtures of identical class conditional distributions. Furthermore,
the label shift framework from these works is non-trivial to generalize
to all settings of DA.

In this paper, we address the issues of the previous works by defining
a novel label shift framework via Wasserstein (WS) distance for a
general DA setting that takes into account the data shift between
two domains. We then develop a theory for our proposed label shift
based on useful properties of WS distance, such as its horizontal
view, numeric stability, and continuity \citep{pmlr-v70-arjovsky17a}.
We refer readers to \cite{santambrogio2015optimal,villani2008optimal,peyre2019computational}
for a comprehensive knowledge body of optimal transport theory and
WS distance, and Appendix \ref{sec:Notations} for necessary backgrounds
of WS for this work. %\vspace{-2mm}


\subsection{Label Shift via Wasserstein Distance \label{sec:label_shift_optimal_transport}
}

To facilitate our ensuing discussion, we assume that the source (S)
and target (T) distributions $\mathbb{P}^{S}$ and $\mathbb{P}^{T}$
are atomless distributions on Polish spaces. Therefore, there exists
a transformation $L:\mathcal{X}^{T}\goto\mathcal{X}^{S}$ such that
$L\#\mathbb{P}^{T}=\mathbb{P}^{S}$ \citep{villani2008optimal}. Given
that mapping $L$, a data example $\bx^{T}\sim\mathbb{P}^{T}$ with
the ground-truth prediction probability $f^{T}\left(\bx^{T}\right)$
corresponds to another data example $\bx^{S}=L\left(\bx^{T}\right)\sim\mathbb{P}^{S}$
with the ground-truth prediction probability $f^{S}\left(\bx^{S}\right)$.
Hence, it induces a label mismatch loss 
\[
d_{Y}\left(f^{T}\left(\bx^{T}\right),f^{S}\left(\bx^{S}\right)\right)=d_{Y}\left(f^{T}\left(\bx^{T}\right),f^{S}\left(L\left(\bx^{T}\right)\right)\right),
\]
where $d_{Y}$ is a given metric over $\mathcal{Y}_{\Delta}$. Based
on that concept, the label shift between the source and target domains
induced by the transformation $L$ can be defined as 
\begin{align}
LS\left(S,T;L\right):=\mathbb{E}_{\mathbb{P}^{T}}\left[d_{Y}\left(f^{T}\left(\bx^{T}\right),f^{S}\left(L\left(\bx^{T}\right)\right)\right)\right].
\end{align}
By finding the optimal mapping $L$, the label shift between two domains
is defined as follows.
\begin{defn}
\label{def:label_shift} Let $d_{Y}$ be a metric over the simplex
$\mathcal{Y}_{\Delta}$. The label shift between the source and the
target domains is defined as the infimum of the label shift induced
by all valid transformations $L$: {\footnotesize{}
\begin{equation}
LS\left(S,T\right):=\inf_{L:L\#\mathbb{P}^{T}=\mathbb{P}^{S}}LS\left(S,T;L\right)=\inf_{L:L\#\mathbb{P}^{T}=\mathbb{P}^{S}}\mathbb{E}_{\mathbb{P}^{T}}\left[d_{Y}\left(f^{T}\left(\bx^{T}\right),f^{S}\left(L\left(\bx^{T}\right)\right)\right)\right].\label{eq:ls_def}
\end{equation}
} We give an illustration for Definition~\ref{def:label_shift} in
Figure \ref{fig:motivation_LS}. The label shift in Eq.~(\ref{eq:ls_def})
suggests finding the optimal transformation $L^{*}$ to optimally
align the source and target domains with a minimal label mismatch.
\end{defn}

\textbf{Properties of label shift via Wasserstein distance:} To show
the connection between the aforementioned label shift and optimal
transport, we introduce two ways of calculating the label shift via
Wasserstein distance.
\begin{prop}
\label{thm:label_shift} (i) Denote by $\mathbb{P}_{f^{S}}^{S}$ the
joint distribution of $\left(\bx,f^{S}\left(\bx\right)\right)$, where
$\bx\sim\mathbb{P}^{S}$, and $\mathbb{P}_{f^{T}}^{T}$ the joint
distribution of $\left(\bx,f^{T}\left(\bx\right)\right)$, where $\bx\sim\mathbb{P}^{T}$.
Then, we have: $LS\left(S,T\right)=\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right).$

%\vspace{-1mm}
 (ii) Let $\mathbb{P}_{f^{S}}$ and $\mathbb{P}_{f^{T}}$ be the push-forward
measures of $\mathbb{P}^{S}$ and $\mathbb{P}^{T}$ via $f^{S}$ and
$f^{T}$ respectively, i.e., $\mathbb{P}_{f^{S}}=f^{S}\#\mathbb{P}^{S}$
and $\mathbb{P}_{f^{T}}=f^{T}\#\mathbb{P}^{T}$. Then, we have: $LS\left(S,T\right)=\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}}\right).$%\vspace{-3mm}
\end{prop}

The results of Proposition ~\ref{thm:label_shift} indicate that
we can compute the label shift via the Wasserstein distance on the
simplex. For example, when $d_{Y}(y,y')=\|y-y'\|_{p}^{p}$, the label
shift can be computed via the familiar $\mathcal{W}_{p}$ distance
between $\mathbb{P}_{f^{S}}$ and $\mathbb{P}_{f^{T}}$, i.e., $LS(S,T)=\mathcal{W}_{p}^{p}(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}})$.
Note that $\mathcal{W}_{d}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right)$
with $d=\lambda d_{X}+d_{Y}$ was studied in \cite{courty2017joint}
for proposing a DA method that can mitigate both label and data shifts.
However, the concept label shift was not characterized and defined  explicitly
in that work. Moreover, our motivation and theory development in this
work are different and independent from \citep{courty2017joint}.
To give a better understanding of our label shift definition, we now
present some bounds for it in general and specific cases. 
\begin{prop}
\label{proposition:properties_labelshift} Denote by $p_{Y}^{S}=(p_{Y}^{S}(y))_{y=1}^{M}$
and $p_{Y}^{T}=(p_{Y}^{T}(y))_{y=1}^{M}$ the marginal distributions
of the source and target domain labels, i.e., $p_{Y}^{S}(y)=\int_{\mathcal{X}^{S}}p^{S}(x,y)dx$
and $p_{Y}^{T}(y)=\int_{\mathcal{X}^{T}}p^{T}(x,y)dx$. For $d_{Y}(y,y')=\|y-y'\|_{p}^{p}$
when $p\geq1$, the following holds:

(i) $\mathcal{L}\left(h^{T},f^{T},\mathbb{P}^{T}\right)\leq LS\left(S,T\right)+\mathcal{L}\left(h^{S},f^{S},\mathbb{P}^{S}\right)+\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)+const$
where the constant can be viewed as a reconstruction term: $\sup_{L,K:L\#\mathbb{P}^{T}=\mathbb{P}^{S},K\#\mathbb{P}^{S}=\mathbb{P}^{T}}\mathbb{E}_{\mathbb{P}^{T}}\left[d_{Y}\left(f^{T}\left(K\left(L\left(\bx\right)\right)\right),f^{T}\left(\bx\right)\right)\right]$; 

(ii) $LS(S,T)\geq\|p_{Y}^{S}-p_{Y}^{T}\|_{p}^{p}$;

(iii) In the setting that $\mathbb{P}^{S}$ and $\mathbb{P}^{T}$
are mixtures of well-separated Gaussian distributions, i.e., $p^{a}(\bx)=\sum_{y=1}^{M}p^{a}(y)\mathcal{N}(\bx|\mu_{y}^{a},\Sigma_{y}^{a})$
with $\|\mu_{y}^{a}-\mu_{y'}^{a}\|_{2}\geq D\times\max\{\|\Sigma_{y}^{a}\|_{op}^{1/2},\|\Sigma_{y'}^{a}\|_{op}^{1/2}\}\,\forall\,a\in\{S,T\},y\neq y'$,
in which $\|\cdot\|_{op}$ denotes the operator norm and $D$ is sufficiently
large, we have 
\begin{equation}
\left|LS(S,T)-\mathcal{W}_{p}^{p}(\mathbb{P}_{Y}^{S},\mathbb{P}_{Y}^{T})\right|\leq\epsilon(D),
\end{equation}
where $\epsilon(D)$ is a small constant depending on $D,p_{Y}^{S},p_{Y}^{T},(\Sigma_{y}^{S},\Sigma_{y}^{T})_{y=1}^{M}$,
and it goes to 0 as $D\to\infty$. 
\end{prop}

A few comments on Proposition~\ref{proposition:properties_labelshift}
are in order. The\emph{ inequality in (i) }bounds the target loss
by the source loss and the label shift. Though this inequality has
the same form as those in \citep{Mansour2009,Ben-David:2010,redko2017theoretical,zhang19_theory,cortes2019adaptation},
the label shift in our inequality is more reasonably expressed. The
\emph{inequality in (ii)} reads that the \emph{marginal label shift}
$\|p_{Y}^{S}-p_{Y}^{T}\|_{p}^{p}$ is a lower bound of our label shift.
Therefore, the label shift induced by the best transformation $L^{*}$
can not be less than this quantity. A direct consequence is that $LS(S,T)=0$
implies $p^{S}(y)=p^{T}(y)$, for all $y\in[M]$ (no label shift).
Finally, the \emph{inequality in (iii)} shows that when the classes
are well-separated, the label shift will almost achieve the lower
bound in the first inequality, which implies its tightness. The key
step in the proof is proving that $\mathbb{P}_{f^{S}}$ and $\mathbb{P}_{f^{T}}$
will be concentrated around the vertices and it is also provable for
sub-Gaussian distributions with some extra work. The bound gives a
simple way to estimate the label shift in this scenario: instead of
measuring the Wasserstein distance $\mathcal{W}(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}})$
on the simplex $\mathcal{Y}_{\Delta}$, we only need to measure the
Wasserstein distance between the vertices equipped with the masses
$p_{Y}^{S}$ and $p_{Y}^{T}$. The first experiment in Section \ref{subsec:label_shift_estimate}
also supports this finding.

Our label shift formulation can also serve as a tool to elaborate
other aspects of DA, as we will see below.

\textbf{Minimizing data shift while ignoring label shift can hurt
the prediction on test set:} Consider two classifiers on the source
and target domains $h^{S}=h\circ g^{S}$ and $h^{T}=h\circ g^{T}$
where $g^{S}:\mathcal{X}^{S}\goto\mathcal{Z}$, $g^{T}:\mathcal{X}^{T}\goto\mathcal{Z}$
are the source and target feature extractors, and $h:\mathcal{Z}\goto\mathcal{Y}_{\simplex}$
with $h\in\mathcal{H}$. We define a new metric $d_{Z}$ with respect
to the family $\mathcal{H}$ as follows: 
\[
d_{Z}\left(\bz_{1},\bz_{2}\right)=\sup_{h\in\mathcal{H}}d_{Y}\left(h\left(\bz_{1}\right),h\left(\bz_{2}\right)\right),
\]
where $\bz_{1}$ and $\bz_{2}$ lie on the latent space $\mathcal{Z}$.
The necessary (also sufficient) condition under which $d_{Z}$ is
a proper metric on the latent space (see the proof in Appendix \ref{sec:proof_key_results})
is realistic and not hard to be satisfied (e.g., the family $\mathcal{H}$
contains any bijection). We now can define a Wasserstein distance
$W_{d_{Z}}$ that will be used in the development of Theorem~\ref{thm:bound_py_diff}. 
\begin{thm}
\label{thm:bound_py_diff} With regard to the latent space $\mathcal{Z}$,
we can upper-bound the label shift as 
\begin{align*}
LS\left(S,T\right)\leq\mathcal{L}\left(h^{S},f^{S},\mathbb{P}^{S}\right)+\mathcal{L}\left(h^{T},f^{T},\mathbb{P}^{T}\right)+\mathcal{W}_{d_{Z}}\left(g^{S}\#\mathbb{P}^{S},g^{T}\#\mathbb{P}^{T}\right).
\end{align*}
%\vspace{-3mm}
\end{thm}

Theorem \ref{thm:bound_py_diff} indicates a trade-off of learning
domain-invariant representation by forcing $g^{S}\#\mathbb{P}^{S}=g^{T}\#\mathbb{P}^{T}$
(e.g., $\min\,\mathcal{W}_{d_{Z}}\left(g^{S}\#\mathbb{P}^{S},g^{T}\#\mathbb{P}^{T}\right)$).
It is evident that if the label shift between domains is significant,
because $\mathcal{L}\left(h^{S},f^{S},\mathbb{P}^{S}\right)$ can
be trained to be sufficiently small, learning domain-invariant representation
by minimizing $\mathcal{W}_{d_{Z}}\left(g^{S}\#\mathbb{P}^{S},g^{T}\#\mathbb{P}^{T}\right)$
leads to a hurt in the performance of the target classifier $h^{T}$
on the target domain. Similar theoretical result was discovered in
\cite{zhao2019learning} for the binary classification (see Theorem
4.9 in that paper). However, our theory is developed based on our
label shift formulation in a more general multi-class classification
setting and uses WS distance rather than Jensen-Shannon (JS) distance
\citep{JS_distance} as in \cite{zhao2019learning} for which the advantages of WS distance over JS distance
have been thoughtfully discussed in \cite{pmlr-v70-arjovsky17a}.

\textbf{Label shift under different settings of DA:} An advantage
of our method is that it can measure the label shift under various
DA settings (i.e., open-set, partial-set, and universal DA). Doing
this task is not straight-forward using other label shift methods.
For example, if there is a label that appears in a domain but not
in the other, it is not meaningful to measure the ratio between the
marginal distribution of this label as in~\cite{NEURIPS2020_219e0524}. 

In what follows, we elaborate our label shift in those settings. Particularly,
we provide some lower bounds for it, implying that the label shift
is higher if there is label mismatch between two domains. Recall that
when the source and target domains do not have the same number of
labels, we can extend $f^{S}$ and $f^{T}$ to be functions taking
values on $\mathcal{Y}_{\Delta}$ by filling $0$ for the missing
labels. For the sake of presenting the results, let $\mathcal{Y}_{S}\cap\mathcal{Y}_{T}=\{1,\dots,C\}$
be the common labels of two domains, $\mathbb{Q}_{S}$ the marginal
of $\mathbb{P}_{f_{S}}$ and $\mathbb{Q}_{T}$ the marginal of $\mathbb{P}_{f_{T}}$
on the first $(C-1)$ dimensions. $\mathbb{Q}_{S\setminus T}$ denotes
the marginal of $\mathbb{P}_{f_{S}}$ in the space of variables having
labels $\mathcal{Y}_{S}\setminus\mathcal{Y}_{T}$ and $\mathbb{Q}_{T\setminus S}$
denotes the marginal of $\mathbb{P}_{f_{T}}$ in the space of variables
having labels $\mathcal{Y}_{S}\setminus\mathcal{Y}_{T}$.
\begin{thm}
\label{thm:label_shift_setting}Assume that $d_{Y}(y,y')=\|y-y'\|_{p}^{p}$.
Then, the following holds:

i) For the partial-set setting (i.e., $\mathcal{Y}^{T}\subset\mathcal{Y}^{S}$),
we obtain 
\begin{equation}
LS(S,T)\geq W_{p}^{p}(\mathbb{Q}_{S},\mathbb{Q}_{T})+\mathbb{E}_{X\sim\mathbb{Q}_{S\setminus T}}\left[\norm X_{p}^{p}\right].\label{eq:partial_bound}
\end{equation}

ii) For the open-set setting (i.e., $\mathcal{Y}^{S}\subset\mathcal{Y}^{T}$),
we obtain 
\begin{equation}
LS(S,T)\geq W_{p}^{p}(\mathbb{Q}_{S},\mathbb{Q}_{T})+\mathbb{E}_{X\sim\mathbb{Q}_{T\setminus S}}\left[\norm X_{p}^{p}\right].\label{eq:open_set_bound}
\end{equation}

iii) For the universal setting (i.e., $\mathcal{Y}^{T}\subsetneq\mathcal{Y}^{S}$
and $\mathcal{Y}^{S}\subsetneq\mathcal{Y}^{T}$), we have 
\begin{equation}
LS(S,T)\geq W_{p}^{p}(\mathbb{Q}_{S},\mathbb{Q}_{T})+\mathbb{E}_{X\sim\mathbb{Q}_{T\setminus S}}\left[\norm X_{p}^{p}\right]+\mathbb{E}_{Y\sim\mathbb{Q}_{S\setminus T}}\left[\norm Y_{p}^{p}\right].\label{eq:universal_bound}
\end{equation}
\end{thm}

%\vspace{-1mm}
 Theorem \ref{thm:label_shift_setting} reveals that the label shifts
for the partial-set, open-set, or universal DA settings are higher
than the vanilla closed-set setting due to the missing and unmatching
labels of two domains (see Section \ref{subsec:label_shift_estimate}). Our theory also implicitly
indicates that by setting appropriate weights for source and target
examples (i.e., low weights for the examples with missing and unmatching
labels), we can deduct label shift by reducing the second term of
lower-bounds in Eqs.~\eqref{eq:partial_bound}, \eqref{eq:open_set_bound},
and \eqref{eq:universal_bound} to mitigate the negative transfer
\citep{cao2019_partial}. We leave this interesting investigation
to our future work. Moreover, further analysis can be found in Appendix
\ref{sec:proof_remaining_results}. 


==> conclusion.tex <==
In this paper, we study label shift between the source and target
domains in a general DA setting. Our main workaround is to consider
valid transformations transporting the target to source domains allowing
us to align the source and target examples and rigorously define the
label shift between two domains. We then connect the proposed label
shift to optimal transport theory and develop further theory to inspect
the properties of DA under various DA settings (e.g., closed-set,
partial-set, open-set, or universal setting). Furthermore inspired
from theory development, we propose\emph{ }\textbf{\emph{L}}\emph{abel
and }\textbf{\emph{D}}\emph{ata Shift }\textbf{\emph{R}}\emph{eduction
via }\textbf{\emph{O}}\emph{ptimal }\textbf{\emph{T}}\emph{ransport}
(LDROT) which can mitigate data and label shifts simultaneously. We
conduct comprehensive experiments to verify our theoretical findings
and compare LDROT against state-of-the-art baselines to demonstrate
its merits. 

%\textbf{Reproducibility Statement: }Source codes for our experiments are  provided in the supplementary of the paper. The details of experimental settings, computational infrastructure, and other used public libraries are given in the supplementary material. All datasets that we used in the paper are published and they are easy to find in the Internet.

%\textbf{Ethics Statement: } Given the nature of the work, we do not foresee any negative societal and ethical impacts of the work.

==> experiments.tex <==

\subsection{Experiments of theoretical part \label{subsec:label_shift_estimate}}

\textbf{Label shift estimation:} In this experiment, we show how to
evaluate the label shift if we know the labeling mechanisms of the
source and target domains. We consider SVHN as the source domain and
MNIST as the target domain. These two datasets have ten categorical
labels which stand for the digits in $\mathcal{Y}=\left\{ 0,1,...,9\right\} $.
Additionally, for each source or target example $\bx$, the ground-truth
label of $\bx$ is a categorical label in $\mathcal{Y}=\left\{ 0,1,...,9\right\} $.
Since these labels have good separation, from part (iii) of Proposition~\ref{proposition:properties_labelshift},
we can choose $f^{S}\left(\bx\right)$ and $f^{T}\left(\bx\right)$
as one-hot vectors on the simplex $\mathcal{Y}_{\simplex}$. Therefore,
$\mathbb{P}_{f^{S}}$ and $\mathbb{P}_{f^{T}}$ are two discrete distributions
over one-hot vectors representing the categorical labels, wherein
each categorical label $y\in\left\{ 0,...,9\right\} $ corresponds
to the one-hot vector $\bone_{y+1}=\left[0,..,0,1_{y+1},0,...,0\right]$.
The label shift between SVHN and MNIST is estimated by either $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right)$
or $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}}\right)$,
where $d_{Y}$ is chosen as $L^{1}$ distance. More specifically,
$\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}}\right)$
is evaluated accurately via linear programming\footnote{\url{https://pythonot.github.io/all.html}},
while estimating $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right)$
using the entropic regularized dual form $\mathcal{W}_{d_{Y}}^{\epsilon}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right)$
with $\epsilon=0.1$~\citep{stochastic_ws}. Moreover, to visualize
the precision when using a probabilistic labeling mechanism to estimate
the label shift, we train two probabilistic labeling functions $h^{S}$
and $h^{T}$ by minimizing the cross-entropy loss with respect to
$f^{S}$ and $f^{T}$respectively and subsequently estimate $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}},\mathbb{P}_{h^{T}}\right)$
using the entropic regularized dual form $\mathcal{W}_{d_{Y}}^{\epsilon}\left(\mathbb{P}_{h^{S}}^{S},\mathbb{P}_{h^{T}}^{T}\right)$
with $\epsilon=0.1$. Note that the prediction probabilities of $h^{S}$
and $h^{T}$ are now the points on the simplex $\mathcal{Y}_{\simplex}$.

We compute the label shift for four DA settings including the closed-set,
partial-set, open-set, and universal settings. As shown in Figure
\ref{fig:label_shift_estimation}, for all DA settings, the blue lines
estimating $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}}^{S},\mathbb{P}_{f^{T}}^{T}\right)$
and the green lines estimating $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{h^{S}},\mathbb{P}_{h^{T}}\right)$
along with batches tend to approach the red lines evaluating $\mathcal{W}_{d_{Y}}\left(\mathbb{P}_{f^{S}},\mathbb{P}_{f^{T}}\right)$
accurately, which illustrates the result of part (iii) in Proposition~\ref{proposition:properties_labelshift}.
We also observe that the label shifts of partial-set, open-set, and
universal settings are higher than the closed-set setting as discussed
in Theorem \ref{thm:label_shift_setting}.

\vspace{0.5 em}
\noindent
\textbf{Implication on target performance:} In this experiment, we
demonstrate that the theoretical finding of Theorem \ref{thm:bound_py_diff}
indicating that forcing learning domain-invariant representations
hurts the target performance. We train a classifier $h^{ST}=g\circ h$,
where $g$ is a feature extractor and $h$ is a classifier on top
of latent representations by solving $\min_{g,h}\{\mathcal{L}\left(h^{ST},f^{S},\mathbb{P}^{S}\right)+0.1\times\mathcal{W}_{L^{1}}^{\epsilon}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)\}$
where $\mathcal{W}_{L^{1}}^{\epsilon}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)$
is used to estimate $\mathcal{W}_{L^{1}}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)$
for learning domain-invariant representations on the latent space.
We conduct the experiments on the pairs A$\rightarrow$W (Office-31)
and P$\rightarrow$I (ImageCLEF-DA) in which we measure the WS data
shift on the latent space $\mathcal{W}_{L^{1}}^{\epsilon}\left(g\#\mathbb{P}^{S},g\#\mathbb{P}^{T}\right)$,
and the source and target accuracies. As shown in Figure \ref{fig:target_performance_hurt},
along with the training process, while the WS data shift on the latent
space consistently decreases (i.e., the latent representations become
more domain-invariant), the source accuracies get saturated, but the
target accuracies get hurt gradually. 
\begin{figure}[!t]
%\vspace{-3mm}
 \centering{}\includegraphics[width=0.5\textwidth]{figures/AW_hurting_target_acc}~~~~~~~~~\includegraphics[width=0.5\textwidth]{figures/PI_hurting_target_acc}
%\vspace{-3mm}
 \caption{Illustration on target performance to show that forcing learning domain-invariant
representations can hurt the target performance. Left: A$\rightarrow$W
(Office-31). Right: P$\rightarrow$I (ImageCLEF-DA). \label{fig:target_performance_hurt}}
%\vspace{-6mm}
 
\end{figure}
%\vspace{-3mm}
 

\subsection{Experiments of LDROT on real-world datasets}

We conduct the experiments on the real-world datasets: Digits, Office-31,
Office-Home, and ImageCLEF-DA to compare our LDROT to the state-of-the-art
baselines, especially OT-based ones DeepJDOT \citep{damodaran2018deepjdot},
SWD \citep{chenyu2019swd}, DASPOT \citep{yujia2019onscalable}, ETD
\cite{li2020enhanceOT}, and RWOT \citep{xu2020reliable}. Due to
the space limit, we show the results for Office-31 and Office-Home
in Tables \ref{tab:office31-dataset-1} and \ref{tab:office-home dataset},
while \emph{other results, parameter settings, and network architectures}
can be found in Appendix \ref{sec:additional_exps}. The experimental
results indicate that our proposed method outperforms the baselines.
\begin{table}[t!]
\centering{}\caption{Classification accuracy (\%) on Office-Home dataset for unsupervised
DA (ResNet-50).\label{tab:office-home dataset}}
\resizebox{0.95\textwidth}{!}{\centering\setlength{\tabcolsep}{2pt}%%
\begin{tabular}{cccccccccccccc}
\hline 
Method  & Ar$\rightarrow$Cl  & Ar$\rightarrow$Pr  & Ar$\rightarrow$Rw  & Cl$\rightarrow$Ar  & Cl$\rightarrow$Pr  & Cl$\rightarrow$Rw  & Pr$\rightarrow$Ar  & Pr$\rightarrow$Cl  & Pr$\rightarrow$Rw  & Rw$\rightarrow$Ar  & Rw$\rightarrow$Cl  & Rw$\rightarrow$Pr  & Avg\tabularnewline
\hline 
ResNet-50 \citep{he2016resnet}  & 34.9  & 50.0  & 58.0  & 37.4  & 41.9  & 46.2  & 38.5  & 31.2  & 60.4  & 53.9  & 41.2  & 59.9  & 46.1\tabularnewline
DANN \citep{ganin2016domain}  & 43.6  & 57.0  & 67.9  & 45.8  & 56.5  & 60.4  & 44.0  & 43.6  & 67.7  & 63.1  & 51.5  & 74.3  & 56.3\tabularnewline
CDAN \citep{long2018cdan}  & 50.7  & 70.6  & 76.0  & 57.6  & 70.0  & 70.0  & 57.4  & 50.9  & 77.3  & \textbf{70.9}  & 56.7  & 81.6  & 65.8\tabularnewline
TPN \citep{pan2019tpn}  & 51.2  & 71.2  & 76.0  & 65.1  & 72.9  & 72.8  & 55.4  & 48.9  & 76.5  & \textbf{70.9}  & 53.4  & 80.4  & 66.2\tabularnewline
SAFN \cite{xu2019sfan}  & 52.0  & 71.7  & 76.3  & 64.2  & 69.9  & 71.9  & 63.7  & 51.4  & 77.1  & \textbf{70.9}  & 57.1  & 81.5  & 67.3\tabularnewline
DeepJDOT \citep{damodaran2018deepjdot}  & 48.2  & 69.2  & 74.5  & 58.5  & 69.1  & 71.1  & 56.3  & 46.0  & 76.5  & 68.0  & 52.7  & 80.9  & 64.3\tabularnewline
ETD \citep{li2020enhanceOT}  & 51.3  & 71.9  & \textbf{85.7}  & 57.6  & 69.2  & 73.7  & 57.8  & 51.2  & 79.3  & 70.2  & 57.5  & 82.1  & 67.3\tabularnewline
RWOT \citep{xu2020reliable}  & 55.2  & 72.5  & 78.0  & 63.5  & 72.5  & 75.1  & 60.2  & 48.5  & 78.9  & 69.8  & 54.8  & 82.5  & 67.6\tabularnewline
\hline 
\textbf{LDROT}  & \textbf{57.4}  & \textbf{79.6}  & 82.5  & \textbf{67.2}  & \textbf{79.8}  & \textbf{80.7}  & \textbf{66.5}  & \textbf{53.3}  & \textbf{82.5}  & \textbf{70.9}  & \textbf{57.4}  & \textbf{84.8}  & \textbf{71.9}\tabularnewline
\hline 
\end{tabular}}%\vspace{-4mm}
 
\end{table}
%\vspace{-2mm}


\subsection{Ablation Study for LDROT}

%\vspace{-1mm}
 We conduct comprehensive ablation studies to investigate the behavior
of our LDROT. Due to the space limit, we leave to the ablation and
analytic studies to Appendix \ref{subsec:Ablation-studies}.


==> introduction.tex <==
The remarkable success of deep learning can be largely attributed
to computational power advancement and large-scale annotated datasets.
However, in many real-world applications such as medicine and autonomous
driving, labeling a sufficient amount of high-quality data to train
accurate deep models is often prohibitively labor-expensive, error-prone,
and time-consuming. Domain adaptation (DA) or transfer learning has
emerged as a vital solution for this issue by transferring knowledge
from a label-rich domain (a.k.a. source domain) to a label-scarce
domain (a.k.a. target domain). Along with practical DA methods \citep{Ganin2015,TzengHDS15,long2015,shu2018a,french2018selfensembling}
which have achieved impressive performance on real-world datasets,
the theoretical results \citep{Mansour2009,Ben-David:2010,redko2017theoretical,zhang19_theory,cortes2019adaptation}
are abundant to provide rigorous and insightful understanding of various
aspects of transfer learning.

For domain adaptation, the source domain consists of the data distribution
$\mathbb{P}^{S}$ with the density $p^{S}$, and the unknown ground-truth
labeling function $f^{S}$ assigning label $y$ to source data $x$,
whilst these are $\mathbb{P}^{T}$, $p^{T}$, and $f^{T}$ for the
target domain, respectively. Moreover, while the data shift can be
characterized as a divergence between $\mathbb{P}^{S}$ and $\mathbb{P}^{T}$
\citep{Mansour2009,Ben-David:2010,redko2017theoretical,zhang19_theory,cortes2019adaptation},
the label shift in these works is commonly characterized as $\mathbb{E}_{\mathbb{P}^{T}}\left[\left|f^{S}\left(\bx\right)-f^{T}\left(\bx\right)\right|\right]$
or $\mathbb{E}_{\mathbb{P}^{S}}\left[\left|f^{S}\left(\bx\right)-f^{T}\left(\bx\right)\right|\right]$
in which the binary classification with deterministic labeling functions
$f^{S}\left(\cdot\right),f^{T}\left(\cdot\right)\in\left\{ 0,1\right\} $
was examined. Additionally, although this label shift term has occurred
in the theoretical analysis of \cite{Mansour2009,Ben-David:2010,redko2017theoretical,zhang19_theory,cortes2019adaptation},
it is restricted in considering the shift between $f^{S}\left(\bx\right)$
and $f^{T}\left(\bx\right)$ at the same data $\bx$, which ignores
the data shift between $\mathbb{P}^{S}$ and $\mathbb{P}^{T}$. This
limitation is illustrated in Figure \ref{fig:motivation_LS}. In particular,
for a white/square point $\bx$ drawn from the target domain as in
$\mathbb{E}_{\mathbb{P}^{T}}\left[\left|f^{S}\left(\bx\right)-f^{T}\left(\bx\right)\right|\right]$,
the source labeling function $f^{S}$ cannot give reasonable prediction
probabilities for $\bx$, hence leading to inaccurate $\left|f^{S}\left(\bx\right)-f^{T}\left(\bx\right)\right|$. 

Label shift has also been examined in an anti-causal setting \citep{pmlr-v80-lipton18a,unified_labelshift_NEURIPS2020},
wherein an intervention on \emph{$p(y)$} induces the shift, but the
process generating $\bx$ given $y$ is fixed, i.e., $p^{S}\left(\bx\mid y\right)=p^{T}\left(\bx\mid y\right)$.
Although this setting is useful in some specific scenarios (e.g.,
a diagnostic problem in which diseases cause symptoms), it is not
sufficiently powerful to cope with a general DA setting. Particularly,
in an anti-causal setting, the source and target data distributions
(i.e., $p^{S}\left(\bx\right)$ and $p^{T}\left(\bx\right)$) are
just simply two different mixtures of the class conditional distributions
$p^{S}\left(\bx\mid y\right)=p^{T}\left(\bx\mid y\right)$, hence
sharing the same support set. This is certainly far from a general
DA setting in which both \emph{data shift}: $p^{S}\left(\bx\right)\neq p^{T}\left(\bx\right)$
with arbitrarily separated support sets and \emph{non-covariate shift}:
$p^{S}\left(y\mid\bx\right)\neq p^{T}\left(y\mid\bx\right)$ appear. 

\textbf{Contribution.} In this paper, we study the label shift for
a general domain adaptation setting in which we have both \emph{data
shift}: $p^{S}\left(\bx\right)\neq p^{T}\left(\bx\right)$ with arbitrarily
separated support sets and \emph{non-covariate shift}: $p^{S}\left(y\mid\bx\right)\neq p^{T}\left(y\mid\bx\right)$.
More specifically, our developed label shift is applicable to a general
DA setting with a data shift between two domains and two totally
different labeling functions (i.e., we cannot use $f^{S}$ to predict
accurately target examples and vice versa). To define the label shift
between two given domains, we utilize transformation $L$ to transport
the target to the source data distributions (i.e., $L\#\mathbb{P}^{T}=\mathbb{P}^{S}$).
This transformation allows us to align the data of two domains. Subsequently,
the label shift between two domains is defined as the infimum of the
label shift induced by such a transformation with respect to all feasible
transformations. This viewpoint of label shift has a connection to
optimal transport~\citep{santambrogio2015optimal,villani2008optimal,peyre2019computational},
which enables us to develop theory to quantify the label shift for
various DA settings, e.g., anti-causal, closed-set, partial-set, open-set,
and universal settings. Overall, our contributions can be summarized
as follows: 

\textbf{1.} We characterize the label shift for a general DA setting
via optimal transport. From that, we develop a theory to estimate
the label shift for various DA settings and study the trade-off of
learning domain-invariant representations and WS label shift. 

\textbf{2.} Inspired from the theoretical development, we propose
\textbf{\emph{L}}\emph{abel and }\textbf{\emph{D}}\emph{ata Shift
}\textbf{\emph{R}}\emph{eductions via }\textbf{\emph{O}}\emph{ptimal
}\textbf{\emph{T}}\emph{ransport} (LDROT) which aims to mitigate both
data and label shifts. We conduct comprehensive experiments to verify
our theoretical findings and compare the proposed LDROT with the baselines
to demonstrate the favorable performance of our method. 

\textbf{Related works.} Several attempts have been proposed to characterize
the gap between general losses of source and target domains in DA,
notably \citep{Mansour2009,Ben-David:2010,redko2017theoretical,zhang19_theory,cortes2019adaptation}.
\cite{ben2012b,ben2012c,zhang19_theory} study the impossibility
theorems for DA, attempting to characterize the conditions under which
it is nearly impossible to perform transferability between domains.
PAC-Bayesian view on DA using weighted majority vote learning has
been rigorously studied in \cite{ger13,ger16}. Meanwhile, \cite{zhao2019learning,pmlr-v89-johansson19a}
interestingly indicate the insufficiency of learning domain-invariant
representation for successful adaptation. Specifically, \cite{zhao2019learning}
points out the degradation in target predictive performance if forcing
domain invariant representations to be learned while two marginal
label distributions of the source and target domains are overly divergent.
\cite{pmlr-v89-johansson19a} analyzes the information loss of non-invertible
transformations and proposes a generalization upper bound that directly
takes it into account. \cite{pmlr-v139-le21a} employed a transformation
to align two domains and developed theories based on this assumption.
Moreover, label shift has been examined for the anti-causal setting
\cite{pmlr-v80-lipton18a,unified_labelshift_NEURIPS2020}, which
seems not sufficiently realistic for a general DA setting. Optimal
transport theory has been theoretically leveraged with domain adaptation
\citep{courty2017joint}. We compare our proposed LDROT to DeepJDOT
\citep{damodaran2018deepjdot} (a deep DA approach based on the theory
of \citep{courty2017joint}), and other OT-based DDA approaches, including
SWD \citep{chenyu2019swd}, DASPOT \citep{yujia2019onscalable}, ETD
\citep{li2020enhanceOT}, RWOT \citep{xu2020reliable}. Finally, in
\citep{tachet2020domain} , a generator $g$ is said to produce generalized
label shift (GLS) representations if it transports source class conditional
distributions to corresponding target ones. Further theories were
developed to indicate that GLR representations are satisfied if we
enforce clustering structure assumption assisting us in training a
perfect classifier. Evidently, our work which focuses on how to quantify
the label shift between two different domains taking into account
the inherent data shift via optimal transport theory is totally different
form that work in terms of motivation and developed theory.

